New Techniques for Proving Fine-Grained Average-Case Hardness

The recent emergence of fine-grained cryptography strongly motivates developing an average-case analogue of Fine-Grained Complexity (FGC). This paper defines new versions of OV, $k$SUM and zero-$k$-clique that are both worst-case and average-case fine-grained hard assuming the core hypotheses of FGC. We then use these as a basis for fine-grained hardness and average-case hardness of other problems. The new problems represent their inputs in a certain ``factored'' form. We call them ``factored''-OV, ``factored''-zero-$k$-clique and ``factored''-$3$SUM. We show that factored-$k$-OV and factored $k$SUM are equivalent and are complete for a class of problems defined over Boolean functions. Factored zero-$k$-clique is also complete, for a different class of problems. Our hard factored problems are also simple enough that we can reduce them to many other problems, e.g.~to edit distance, $k$-LCS and versions of Max-Flow. We further consider counting variants of the factored problems and give WCtoACFG reductions for them for a natural distribution. Through FGC reductions we then get average-case hardness for well-studied problems like regular expression matching from standard worst-case FGC assumptions. To obtain our WCtoACFG reductions, we formalize the framework of [Boix-Adsera et al. 2019] that was used to give a WCtoACFG reduction for counting $k$-cliques. We define an explicit property of problems such that if a problem has that property one can use the framework on the problem to get a WCtoACFG self reduction. We then use the framework to slightly extend Boix-Adsera et al.'s average-case counting $k$-cliques result to average-case hardness for counting arbitrary subgraph patterns of constant size in $k$-partite graphs...

==> ConstFramework.tex <==


For a variety of detection problems (for example the clique detection problem) they can be solved given a solver for the counting mod two  problem. As an intuition, consider the $k$-clique problem. If we want to distinguish between zero and more than zero cliques we can sub-sample the graph. If we delete enough nodes and edges in a graph with zero cliques we will always find zero mod two cliques. However, in graphs with at least one clique deleting subsets of the vertices and edges has some probability of producing a graph with an odd number of cliques. 

\begin{lemma}
If the worst case counting clique mod $q$ where $q \geq 2$ is any fixed constant integer can be solved in $T_q(n)$ time then worst case detecting clique can be solved in $T_q(n)$ time \cite{??}.
\end{lemma}

Let $q$ be a small prime. 
If solving the counting mod $q$ problem is hard for a problem $P$ and there is a degree $d \leq q/12$ \goodPoly~for the problem $P$, then getting the correct answer for the problem $P$ with probability $1-q^{-d}/3$ is hard when all bits of the input are selected iid at random with probability $1/q$.

Note that if $q$ is constant we can now say that the problem $P$ is hard, even when there is a constant probability of error. But, further note that we no longer can produce any constant probability $\mu$ for the input bits being $1$, we have the specific probability $1/q$. 

Consider the case of $3$-clique to be concrete. The \goodPoly~for counting $3$-clique has degree $3$. So if we choose $q=37>3\cdot 12$, we can say that counting $3$-cliques on $3$-partite \erdosRen~graphs mod $37$ with edge probability $1/37$ with probability greater than $1-\frac{1}{37^{3}\cdot 3}$ requires the same time as detecting $3$-cliques in the worst case (up to constant factors). 

More generically: our framework is implicitly for counting problems. But, if we start by assuming a detection problem is hard, we can say that counting over a small modulus is hard. If the degree of the polynomial is very small then we can make improvements in both the efficiency of the reduction and the implied probability of success needed for algorithms to have lower bounds against them. 

The advantages are more efficient reductions and less stringent requirements on the success probability of the algorithms we get lower bounds against. The downside is that we start with a stronger assumption and require the graphs to have \emph{particular} edge probabilities. We don't, for example, show that $3$-clique is hard to count with constant probability when edges appear with probability $1/2$. 



\xxx{TODO: a version of Lemma \ref{lem:UnifPtoACf}  with roughly $1-1/(12d)^d$ error (really the smallest prime larger than $12d$ when $d>9$).}

\xxx{TODO: a version of Theorem \ref{thm:framework} with roughly $1-1/(12d)^d$ error (really the smallest prime larger than $12d$ when $d>9$).}

\xxx{TODO: a version of Inclusion Edgesclusion where we note that the error can be constant if $k$ is (the thm statement is ready for it). }


\xxx{TODO: Throw all of the above together and you get that clique with $1-1/f(k)$ error is hard. Where $f(k) \approx k^{2k^2}$.  }

==> HowTo.tex <==
We will give a guide for applying the tools and frameworks of this paper. 

\subsection{So You Want to Prove Uniform Average-Case Hardness:\\
How to Use Good Low-Degree Polynomials}

Let $P$ be a problem that takes an $n$ bit input $I$. The uniform average case with probability $\mu$ draws each of the $n$ bits identically and independently where we draw $1$ with probability $\mu$ and $0$ with probability $1-\mu$.

Now, recall the definition of $\gPol{P}$.

\begin{definition}[\goodPoly~Definition \ref{def:goodPoly}]
Let $n$ be the input size of the problem $P$, let $P$ return an integer in the range $[0,p-1]$ where $p$ is a prime and $p < n^c$ for some constant $c$. 
A \emph{\goodPoly} for problem $P$  (\gPol{P})  is a polynomial $f$ over a prime finite field $F_{p}$ where:
\begin{itemize}
    \item There are at most polynomial monomials in $f$.
    \item If $\vec{I} = b_1,\ldots, b_n$, then 
    $f(b_1,\ldots, b_n) = f(\vec{I})=P(\vec{I})$ were $b_i$ will map to either a zero or a one in the prime finite field.
    \item The function $f$ has degree $d = o\left( \lg(n)/\lg\lg(n) \right)$.
    \item the function $f$ is strongly $d$-partite. 
\end{itemize}
\end{definition}

To show that $P$ is hard in the average case find a polynomial $f$ that is a $\gPol{P}$. The most likely hurdle will be the degree (a degree of $o(\lg(n)/\lg\lg(n))$ is quite small). The second mostly likely hurdle will be making your function strongly $d$-partite.  You need to separate the input into $d$ partitions such that every monomial involves exactly one variable from each partition. 

If you manage to construct a $\gPol{P}$, then you can apply Theorem \ref{thm:framework}. This gives the result that a $T(n)$ time algorithm for $P$ in the average-case that succeeds with high enough probability (probability at least $1-1/\omega(\lg^d(n)\lg\lg^d(n))$) implies a $\tO(T(n))$ time algorithm for $P$ in the worst case that succeeds with high probability. 

So, just constructing a $\gPol{P}$ implies a worst-case to average-case self-reduction for the problem $P$. 

We will give some tips for constructing $d$-partite $\gPol(\cdot)$ functions.\\
It is easiest to get the strong $k$-partite structure if you start with a worst-case problem that has the $k$-partite structure. We suggest considering versions of the problem (ideally worst-case equivalent versions) that are $k$-partite. For example, we could consider a version of \fkov[]~that takes a single list as input. This version would allow all $k$ tuples of vectors to be compared. However, this version does not lend itself to a $gk$ partite representation. \\
Another issue is 

\subsection{So You Want to Reduce from a Factored Problem}

==> MatrixMult.tex <==

\newcommand{\MM}{MM}
\newcommand{\MMp}{MM(p)}
\newcommand{\ACMp}{ACMM(p)}
\newcommand{\UACM}{UACMM$^{\mu}$}
\newcommand{\UACMp}{UACMM$^{\mu}$}

\begin{definition}
Matrix Multiplication (\MM) takes as input two $n \times n$ matrices where every entry is in $[-n^c,n^c]$ for some fixed constant $c$. To solve \MM~ one must return the multiplication of the two matrices over the integers. 
\end{definition}
\begin{definition}
Matrix Multiplication (\MMp) takes as input two $n \times n$ matrices where every entry is in $[0,p-1]$. To solve \MMp~ one must return the multiplication of the two matrices over the integers $\mod p$. 
\end{definition}
\begin{definition}
Average-Case Matrix Multiplication Mod p (\ACMp) takes as input two $n \times n$ matrices where every entry is iid selected over $\Unif[1,p-1]$ for some fixed constant $c$. To solve \ACMp~ one must return the multiplication of the two matrices over the integers$\mod p$. 
\end{definition}

\begin{definition}
For simplicity let $D_{\mu}$ be the distribution over $n \times n$
matrices where every entry is chosen to be a one with probability $\mu$ and a zero with probability $1-\mu$.
\end{definition}

\begin{definition}
Uniform Average-Case 0/1 Matrix Multiplication (\UACM) takes as input two $n \times n$ matrices where the input matrices are drawn from $D_{\mu}$. To solve \UACM~ one must return the multiplication of the two matrices over the integers. 
\end{definition}
\begin{definition}
Uniform Average-Case 0/1 Matrix Multiplication Mod p (\UACMp) takes as input two $n \times n$ matrices where the input matrices are drawn from $D_{\mu}$. To solve \UACMp~ one must return the multiplication of the two matrices over the integers$\mod p$. 
\end{definition}

\begin{lemma}
An algorithm which solves \MMp for all $p \in \Theta(\lg(n))$ in time $T(n)$ with implies that \MM is solve able in time $\tO(T(n))$ time.
\label{lem:MMpToMM}
\end{lemma}
\begin{proof}
There are $\Theta(\lg(n)/\lg\lg(n))$ primes of in $[c\lg(n), (c+1)\lg(n)$ when $c$ is a constant using the prime density. So, for a sufficiently large constant $c$ the range $[\lg(n), c\lg(n)]$
contains at least $2k\lg(n)/\lg\lg(n)$ primes $p_1, \cdots, p_{2k\lg(n)/\lg\lg(n)}$. 
Note that $\Pi_{i=1}{2k\lg(n)/\lg\lg(n)}p_i \geq 2n^k$.
By using the Chinese Reminder Theorem on the each element of the output we can solve for its value over the integers $[-n^k,n^k]$ in time $O(\lg^2(n))$, solving for the whole matrix in time $O(\lg^2(n)n^2)$.
\end{proof}

\begin{lemma}
An algorithm which solves \ACMp for all $p \in \Theta(\lg(n))$ in time $T(n)$ with probability $q \geq 8/9$ implies that \MMp is solve able in time $\tO(T(n) +n^2)$ time with probability at least $1-2^{-\lg^2(n)}$.
\label{lem:ACMpToMMp}
\end{lemma}
\begin{proof}
For this we will use the standard proof of average case complexity for Matrix Multiplication, altered to the $\mod p$ setting \cite{?}. 

Consider the input $X$ and $Y$ matrices. Consider two random matrices with every entry picked iid from $\Unif[1,p-1]$, $R_X$ and $R_Y$ now consider the following multiplications:
\begin{align}
    \left(X+R_X \right) \times \left(Y+R_Y\right)&= Z_1\\     \left(R_X \right) \times \left(Y+R_Y\right)&= Z_2\\     \left(X+R_X \right) \times \left(R_Y\right)&= Z_3 \\  \left(R_X \right) \times \left(R_Y\right)&= Z_4
\end{align}
Each multiplication has an input that is iid random. However, the four multiplications are correlated.

Note that $X \times Y = Z_1-Z_2-Z_3+Z_4$. So if all four multiplications are correct, then we can reproduce $X \times Y$. If random multiplications are correct with probability at least $8/9$ then the probability that one of the four multiplications is wrong is at most $4/9$. Thus, the probability we produce the correct $X \times Y$ is at least $5/9$ for every choice of random $R_X$ and $R_Y$. We can repeat with fresh randomly chosen  $R_X$ and $R_Y$ $\lg^3(n)$ times and choose the output matrix that appears the most often to find $X \times Y$ with probability at least $1-2^{\lg^2(n)}$. 
\end{proof}

\begin{lemma}
An algorithm which solves \UACMp for all $p \in \Theta(\lg(n))$ in time $T(n)$ with probability greater than $1-1/\omega(\lg\lg^2(n)\lg^2(n))$ implies that \ACMp is solvable in time $\tO(T(n) +n^2)$ time with probability greater than $8/9$.
\label{lem:UACMpToACMp}
\end{lemma}
\begin{proof}

We will use Corollary \ref{cor:SampleButNoEps} to prove this (note our input size is $n^2$, so the ``n'' of the Lemma is $n^2$). Given an input from \ACMp, matrices $X$ and $Y$, where $p = \Theta(\lg(n))$ we apply the sampling procedure from Corollary \ref{cor:SampleButNoEps} the $\mu$ of the Corollary is the same as our $\mu$. 

Because $\mu$ is constant and $p = \Theta(\lg(n))$, $t = O(\lg(n)\lg\lg(n))$. Thus, the procedure requires $O(n^2 \lg^4(n)\lg\lg^2(n))$ time.  The total variation distance of these new $t$ bit numbers and uniform distribution where every bit is picked iid at random is $1/2$ is $\epsilon = 1/n^{6}$. 

Consider creating $t$ matrices for each of $X$ and $Y$: where $X_i$ and $Y_i$ is the $\{0,1\}$ matrix formed by taking the $i^{th}$ bit of every number in $X$ and $Y$ respectively. For example if $X[j][k]$ is the number represented by bits $b_{t-1},\ldots,b_0$ then $X_i[j][k] =b_i$.

Now consider creating $t^2$ $\{0,1\}$ matrix multiplication instances by taking $X_i$ and $Y_j$ for all $i\in[0,t-1]$ and all $j \in [0,t-1]$. Note that if we have the correct multiplication of all $t^2$ of these instances we can produce a correct multiplication of $X$ and $Y$. Specifically, if $X \times Y = Z$ then $Z[a][b] = \sum_{d \in [1,n]} X[a][d]Y[d][b]$. We can rewrite this as the bit by bit expansion of the multiplication:
$$Z[a][b] = \sum_{d \in [1,n]} \sum_{i,j\in[0,t]} 2^i \cdot 2^j \cdot X_i[a][d]Y_j[d][b].$$
So we can produce $Z$ by summing the matrices $2^{i+j}\left( X_i \times Y_j\right)$ for all $i$ and $j$. We only want to learn $Z \mod p$, so we only need $X_i \mod p$ and $Y_i \mod p$. After doing our calculation we can once again mod by $p$ to get the desired output, $Z_p$. 

We are going to proceed by assuming an algorithm $A$ exists that solves \UACMp~as described in the Lemma. These $t^2$ instances of $X_i$ and $Y_j$ inputs are going to be fed to the the algorithm $A$. If we can solve all $t^2$ instances correctly with probability greater than $q$ then we can solve \ACMp~instances with probability greater than $q-2^{-\lg^2(n)}$ (the $2^{-\lg^2(n)}$ error is introduced by the probability the sampling procedure fails) .

Assume an algorithm $A$ exists which correctly multiplies two matrices with probability at least $1-1/\omega(\lg\lg^2(n)\lg^2(n))$ when the matrices are drawn from $D_{\mu}$. % then it must solve any given group of  $O(\lg\lg^2(n)\lg^2(n))$ instances, even if they are not independent from one another, generated from $D_{\mu}$ with probability at least $1-\frac{1}{\omega(1)}$. 

Any given $X_i$ $Y_j$ input has total variation distance at most $1/n^3$ from $D_{\mu}$. Thus, $A$ must correctly multiply $X_i$  and $Y_j$ with probability at least $1-1/\omega(\lg\lg^2(n)\lg^2(n)) - 1/n^3 = 1-1/\omega(\lg\lg^2(n)\lg^2(n))$ for one given $X_i$ $Y_j$ instance. 

The instances $X_i$ $Y_j$ correlated with other generated instances (notably $X_i$ $Y_{j'}$ and $X_{i'}$ $Y_j$). However, despite this if $A$ fails with probability at most $q$ overall then $A$ must correctly multiply all $t^2$ instances with probability at least $1-qt^2$. Thus $A$ successfully multiplies all $t^2$ instances with probability at least $1-\frac{1}{\omega(1)} \geq 8/9$.

Thus, if $A$ runs in time $T(n)$ and succeeds with probability $1-1/\omega(\lg\lg^2(n)\lg^2(n))$ over instances drawn from $D_{\mu}$, then \ACMp is solvable in time 
$$T(n)t^2 +n^2 \lg^4(n)\lg\lg^2(n) = \tO(T(n) +n^2)$$
with probability greater than 
$$1-\frac{1}{\omega(1)}- 1/n^3 -2^{-\lg^2(n)} = 1-\frac{1}{\omega(1)} \geq 8/9.$$

% We use their result with \eps ~ 1/n^3 so the tvd is super low. 
% Then we multiply bit by bit

\end{proof}

\begin{theorem}
An algorithm which solves \UACMp, for all $p \in \Theta(\lg(n))$ with probability $1-\frac{1}{\omega(\lg^2(n)\lg\lg^2(n))}$ in time $T(n)$ implies that worst case matrix multiplication is solvable in time $\tO \left( n^2 + T(n) \right)$ with probability at least $1-2^{-\lg^(n)}$.
\end{theorem}
\begin{proof}
Using Lemmas \ref{lem:MMpToMM},\ref{lem:ACMpToMMp} and, \ref{lem:UACMpToACMp} we can reduce an algorithm that solves \UACMp~for all $p \in \Theta(\lg(n))$ correctly with probability great than $1-1/\omega(\lg^2(p)\lg^2(n))$ to $MM$. By plugging in $p = \Theta(\lg(n))$ the probability becomes $1-1/\omega(\lg\lg^2(n)\lg^2(n))$, giving us the result above. 
\end{proof}

\begin{corollary}
An algorithm which solves \UACM~with probability $1-\frac{1}{\omega(\lg^2(n)\lg\lg^2(n))}$ in time $T(n)$ implies that worst case matrix multiplication is solvable in time $\tO \left( n^2 + T(n) \right)$.
\end{corollary}
\begin{proof}
If we can solve \UACM~, we solve \UACMp~ for any $p \in \Theta(\lg(n))$ trivially. We can simply take the output of \UACM~and mod by $p$ for any choice of $p \in \Theta(\lg(n))$. This gives us the desired result.
\end{proof}


Note that while the input to these random matrices is $\{0,1\}$ the output matrix has larger values (either up to $[0,n^2]$ or $\mod p$ where $p =\Theta(\lg(n))$). Additionally, note that multiplying these zero-one matrices are as hard as multiplying matrices where every entry is polynomially sized. 

==> OptimalFramework.tex <==
Here we will prove that some improvements to the framework imply the violation of many important hypotheses simultaneously. 

\paragraph{Sparsity:} Getting additional sparsity ``for free'' from the framework would obviously be appealing. However, it would violate many conjectures simultaneously. 

\xxx{TODO: the compressed versions are very happy when we have low sparsity. When you get sparsity low enough our instance size is super small. So we can just brute force all the tiny instances. }

==> abstract-Short.tex <==

\begin{abstract}
In this paper we introduce new techniques for average-case hardness from Fine-Grained Complexity (FGC) hypotheses, 
specifically, computational hypotheses about the running time of  Orthogonal Vectors (OV), CNF-SAT, $3$SUM, All-Pairs Shortest Paths (APSP) and zero-$k$-clique.
We define new problems which are both worst-case and average-case fine-grained hard (under natural distributions) assuming the core hypotheses of FGC, and use them as a basis for fine-grained hardness and average-case hardness of other problems.
The new problems we define look similar to OV, zero-$k$-clique and $3$SUM, but they represent the inputs of the problems in a certain ``factored'' form. We call them ``factored''-OV, ``factored''-zero-$k$-clique and ``factored''-$3$-SUM. 

We show that factored-$k$-OV and factored-$k$-SUM are equivalent and are complete for a certain factored class of problems defined over Boolean functions.
Factored zero-$k$-clique is also complete, for a different class of problems. We show that factored-$k$-OV, factored-$k$SUM and factored zero-$k$-clique require $n^{k-o(1)}$ time if SETH (a FGC hypothesis) is true. We additionally show that factored zero-$3$-clique requires $n^{3-o(1)}$ time if any of SETH, the APSP hypothesis or the $3$-SUM hypothesis are true. 

Our factored problems are hard but also simple enough that we can reduce them to many other problems, e.g. to edit distance, $k$-LCS and versions of  Max-Flow. We further consider counting variants of our factored problems and give worst-case to average-case (WCtoAC) reductions for them for a natural distribution. Through FGC reductions we then get \emph{average-case} hardness for well-studied problems like counting regular expression matchings from standard \emph{worst-case} FGC assumptions. 

To obtain our WCtoAC reductions for factored problems, we formalize the framework of [Boix-Adser{\`{a}} et al. 2019] that was used to give a WCtoAC reduction for counting $k$-cliques.  We define an explicit property of problems such that if a problem has that property one can use the framework on the problem to get a WCtoAC reduction. We then use the framework to slightly extend Boix-Adser{\`{a}} et al.'s WCtoAC counting $k$-cliques reduction to a WCtoAC reduction for arbitrary subgraph patterns of constant size in $k$-partite graphs. 

We give two additional results in average-case FGC. 
First, we show that for a natural distribution, an algorithm that detects a zero-$k$-clique with high enough probability also implies an algorithm that can count zero-$k$-cliques with high probability. 
Second, we give a fast algorithm for counting the number of OV pairs in the most natural distribution of binary vector inputs, where each entry is independently generated from a Bernoulli distribution.  It was already known that detecting OV can be solved quickly over the same distribution [Kane-Williams 2019].

\end{abstract}

==> abstract.tex <==
\begin{abstract}
Fine-grained complexity (FGC) is a vibrant research area with many applications. 
Recent work [Ball et al. 2017, Ball et al. 2018, LaVigne et al. 2019] introduces fine-grained cryptography and strongly motivates developing average-case FGC. Prior work developed worst-case to average-case fine-grained reductions (WCtoACFG) for certain algebraic and counting problems over natural distributions and used them to obtain a limited set of cryptographic primitives [Goldreich-Rothblum 2018, Boix-Adser{\`{a}} et al. 2019, Ball et al. 2017]. 

To obtain stronger cryptographic primitives based on standard FGC assumptions, ideally, one would like to develop WCtoACFG reductions for the core hard problems from FGC, Orthogonal Vectors (OV), CNF-SAT, $3$SUM, All-Pairs Shortest Paths (APSP) and zero-$k$-clique. Unfortunately, it is unclear whether these problems actually are hard for any natural distribution. For instance, it is known that OV can be solved quickly for the most natural distribution of binary vector inputs, where each entry is independently generated from a Bernoulli distribution [Kane-Williams 2019], and in this paper we show that even counting the number of OV pairs has a fast algorithm.  

We introduce new techniques for average-case hardness from FGC assumptions.
We define new problems which are both worst-case and average-case fine-grained hard (under natural distributions) assuming the core hypotheses of FGC, and use them as a basis for fine-grained hardness and average-case hardness of other problems.
The new problems we define look similar to OV, zero-$k$-clique and $3$SUM, but they represent the inputs of the problems in a certain ``factored'' form. We call them ``factored''-OV, ``factored''-zero-$k$-clique and ``factored''-$3$SUM. We show that factored-$k$-OV and factored $k$SUM are equivalent and are complete for a certain factored class of problems defined over Boolean functions.
Factored zero-$k$-clique is also complete, for a different class of problems. 

Our factored problems are also simple enough that we can reduce them to many other problems, e.g. to edit distance, $k$-LCS and versions of  Max-Flow. We further consider counting factored problems and give WCtoACFG reductions for them for a natural distribution. Through FGC reductions we then get \emph{average-case} hardness for well-studied problems like regular expression matching from standard \emph{worst-case} FGC assumptions. 

To obtain our WCtoACFG reductions, we formalize the framework of [Boix-Adser{\`{a}} et al. 2019] that was used to give a WCtoACFG reduction for counting $k$-cliques.  We define an explicit property of problems so that one can use the framework on them. We then use the framework to slightly extend Boix-Adser{\`{a}} et al.'s average-case counting $k$-cliques result to average-case hardness for counting arbitrary subgraph patterns of constant size in $k$-partite graphs. 

The only known fine-grained public-key encryption scheme [LaVigne et al.'20] is based on an average-case hardness hypothesis for the {\em decision} problem, zero-$k$-clique, and the known techniques for building such schemes break down for algebraic/counting problems.
Meanwhile, the WCtoACFG reductions so far have only been for counting problems. To bridge this gap, we show that for a natural distribution, an algorithm that detects a zero-$k$-clique with high enough probability also implies an algorithm that can count zero-$k$-cliques with high probability. This gives hope that the FGC cryptoscheme of [LaVigne et al.'20] can be based on standard FGC assumptions.


%In this paper we explore average case fine grained complexity (ACFGC). 
%Fine-grained complexity (FGC) has allowed us to understand the relationship between the polynomial hardness of many different problems. Average case complexity allows both for the potential of building cryptographic objects and a better understanding of which instances are hard instances of our problems. Ideally we would find worst-case to average case self reductions from the core problems of FGC: orthogonal vectors (OV), $k$-SUM, APSP.   Unfortunately, we don't understand the hard distributions of many of the problems we care about, for example orthogonal vectors. Detecting orthogonal vectors in the average case is easy \cite{ryanAvgCaseOV}. Most ACFGC techniques so far have produced hardness for counting problems. We might hope that the counting versions of these problems would make better targets. However, we show that even counting orthogonal vectors is easy. 

%As the crucial tool we use in this paper we introduce a new kind of problem, a \emph{factored} problem, that has a self reduction that garners average-case lower bounds. 
%We can define factored versions of the core problems of fine-grained complexity. These factored versions are more expressive, indeed the factored version of the zero k clique problem is $n^{k-o(1)}$ hard from \textbf{all three} of the core hypotheses. Additionally, we prove that factored counting zero $3$ clique over the uniform input is \emph{average-case}  $n^{3-o(1)}$ hard from all three of the \emph{worst-case} core hypotheses. Our versions of factored $k$-OV and factored $k$-SUM reduce to each other and are $n^{k-o(1)}$ hard from SETH. Both factored counting $k$-OV and factored counting $k$-SUM are $n^{k-o(1)}$ hard on average over the uniform input from SETH. 

%We additionally give seven problems which reduce from our factored problems. These problems include a sparse graph problem, two dense graph problems, (k+1)-labeled max flow, regular expression matching, $k$-LCS, and edit distance. Notably, we get tight average-case hardness for the counting version of many of these problems, including counting regular expression matching,  from \emph{all} of the worst case assumptions SETH, $3$-SUM and APSP. 

%To get average-case hardness self reductions we generalize the techniques of Andresar et al to produce a framework from which proving these results is easy. 
%We define the properties a ``good low-degree polynomial'' for a problem $P$ needs to have such that $P$ is as hard in the uniform average case as it is in the worst case. By defining these ``good low-degree polynomails'' we are able to create a framework which easily generalizes to many new problems. Notably, we show average-case hardness for our factored problems and for counting arbitrary subgraphs $H$ in  Erd{\H{o}}s-R{\'{e}}nyi graphs. 
%We use this framework to additionally show that counting a subgraph $H$ of size at most $k$ in  Erd{\H{o}}s-R{\'{e}}nyi graphs is as hard as counting $H$ in worst case graphs, which was stated as an open problem in Andresar et al. 

%The worst case to average case reductions in ACFGC tend to require a counting problem in the average case. Previous work build a public key encryption system from the detection version of average case \zkc~assumption with a probability of $0.99$ (note this is regular \zkc~not factored \zkc). 
%We reduce this gap by giving a counting to detection reduction for average case \zkc, but with high probability $1-n^{-\omega(1)}$. But, this result lends credence to the detection assumption on \zkc.  
\end{abstract}


==> ksum.tex <==
If the $k$-sum problem has numbers with $b$ bits, how hard is counting those $k$-sum solutions? 

If $b> (k+\delta)\lg(n)$ for $\delta>0$ then easy.
If $b< (\lceil k/2 \rceil -\delta) \lg(n)$ then easy.

For values in between consider when we have every one with probability $1/\lg(n)$ (roughly). Then most likely numbers are sparse! If you only have $c\lg(n)/\lg\lg(n)$ ones then there are at most $b^{c\lg(n)/\lg\lg(n)}$ numbers. If $b=x \lg(n)$ then this gives us $2^{c \lg(x) \lg(n)}$ numbers. 

\xxx{TODO: argue about hardness when }

==> oldCountToDetect.tex <==
\xxx{TODO: If you can detect e.g. \ksum~on average with numbers picked randomly from $n^k$ range with probability $1-1/n^k$ (or something like that) then, you can solve average case counting \ksum~over any range. If the range is small, then FFT solves counting \ksum~quickly. If the range is large then the total number of solutions isn't very large so we can use the detection algorithm. }

\xxx{TODO: this same general idea applies to \kOV, \ksum, and \ZKC. These problems have the property that as you add more bits per number the number of OVs and zero sums drop. And, there are fast algorithms if the range is sufficiently small.}


\paragraph{\ksum~Counting to Detection}

\xxx{TODO}


\paragraph{\ZKC~Counting to Detection}

\xxx{TODO}

\paragraph{\kOV~Counting to Detection}

\begin{definition}
Let $D_{kov}[b]$ be the uniform average-case instance of \kOV~with $b$ length vectors, formed by picking all $kbn$ bits uniformly at random. All $b$ bits of each of the $n$ vectors in each of the $k$ lists. 

Let $D_{kov}^{(s)}[b]$ be formed by drawing from $D_{kov}[b]$ and conditioning on there being exactly $s$ orthogonal vectors. Otherwise stated, uniformly over all instances with $k$ lists of $n$ vectors of length $b$ with exactly $s$ orthogonal vectors. 
\end{definition}

\begin{lemma}
Let $\alpha>0$ and $\epsilon >0$ be constants. 

A uniform average-case instance of \kOV~with $b=k 2^k (1+\alpha/k) \ln(2) \lg(n)$ length bit vectors can be solved with probability at least $1 - n^{-\alpha}$ in $O(1)$ time. 

A uniform average-case instance of \kOV~with $\ell =(1-\epsilon/k) \lg(n)$ length bit vectors can be solved with probability $1$ in $O(n^{k-\epsilon})$ time. 
\label{lem:ovFastSmallLargeRanges}
\end{lemma}
\begin{proof}
Let us start with $b=k 2^k (1+\alpha/k) \ln(2) \lg(n)$
The probability of $k$ random $b$ length vectors being orthogonal is : $(1-1/2^k)^b\leq e^{-b/2^k}$. By the union bound the probability that there is an orthogonal $k$-tuple is at most $e^{-b/2^k}\cdot n^k$. This says the probability of an orthogonal $k$-tuple is at most $n^{-k}\cdot n^{-\alpha}\cdot n^k$. Thus, the algorithm that simply returns zero as the count succeeds with probability at least $1 - n^{-\alpha}$. 


Next, lets consider the case of $\ell =(1-\epsilon) \lg(n)$. Here there are only $n^{1-\epsilon}$ possible vectors. We can weight each vector by its number of occurrences and brute force solve the problem in time $O(n^{k-\epsilon})$.
\end{proof}

\begin{lemma}
If an instance is drawn from $D_{kov}^{(s)}[b']$ where $b'>b = k 2^k \ln(2) \lg(n)$ then randomly shortening all the vectors by removing a consistent set of indices to length $b$ has probability at least $1/2$ of having exactly $s$ orthogonal vectors. 
\end{lemma}
\begin{proof}
\xxx{TODO: if we have this then we get the next lemma. If we have the next lemma then we can solve the whole thing.}
\end{proof}




\begin{lemma}
Assume you can solve decision \kOV~with $b=k 2^k \ln(2) \lg(n)$ length vectors in time $T(n)$ with probability $1-p_T$ if there is a solution and $1-p_F$ if there is no solution.
Then you can solve decision \kOV~with $b' = b\cdot g >b$ length vectors in time $T(n)$ with probability at least $1-cp_T-(1-1/g)^{c}n^k$ if there is a solution and probability at least $1-cp_F-(1-1/g)^{c}n^k)$ if there is no solution for any positive integer $c$.
\end{lemma}
\begin{proof}

\xxx{TODO: If we can write this kind of thing, then we will be golden}
\end{proof}

\begin{lemma}

\xxx{TODO: Fill $ \delta$ and p. p will be something like $1/n^k$. $\delta$ will be something like $\epsilon \cdot k$}

Given an algorithm for the uniform average-case instance of \kOV~with $b=k 2^k \ln(2) \lg(n)$ length vectors that solves the search problem in time $n^{k - \delta}$ with probability at least $1-p$ we can solve counting uniform average-case instance of \kOV~over any range with probability at least $1-n^{-\epsilon}$ in time $n^{k-\epsilon}$.

For some constant $\epsilon >0$.
\label{lem:ovCounttoDetect}
\end{lemma}
\begin{proof}
Let $\ell$ be the bit length of the vectors of our counting \kOV~instance.

By Lemma \ref{lem:ovFastSmallLargeRanges}, we have that  the condition is already met when $\ell \leq (1-\epsilon/k) \lg(n)$ and when $\ell \geq k 2^k (1+\epsilon/k) \ln(2) \lg(n)$.

So assume $(1-\epsilon/k) \lg(n) <\ell< k 2^k (1+\epsilon/k) \ln(2) \lg(n)$. Let us define $c$ to be $c = \ell/\lg(n)$ for the convenience of math. 

\xxx{TODO: subdivide until the point where the range matches our goal range. If we get a no, don't explore that path. If we get a yes subdivide until we have problems so small we can just brute force anyway. If the range gets to big we can delete random rows. }

\end{proof}

\xxx{TODO: if we can come up with an algorithm for detecting OV on average with high enough prob of success (ryans paper might do this? Unclear as of now.) then, we can solve counting OV faster. If we can solve counting OV fast over all ranges we can say no formula exists with properties we listed for counting OV. This gives a cool gap, no such formula exists for OV (given k-OV is true), but one does for compressed OV. Anyway! Cool things. }
